Treatment Heterogeneity for Survival Outcomes

Estimation of conditional average treatment effects (CATEs) plays an essential role in modern medicine by informing treatment decision-making at a patient level. Several metalearners have been proposed recently to estimate CATEs in an effective and flexible way by re-purposing predictive machine learning models for causal estimation. In this chapter, we summarize the literature on metalearners and provide concrete guidance for their application for treatment heterogeneity estimation from randomized controlled trials' data with survival outcomes. The guidance we provide is supported by a comprehensive simulation study in which we vary the complexity of the underlying baseline risk and CATE functions, the magnitude of the heterogeneity in the treatment effect, the censoring mechanism, and the balance in treatment assignment. To demonstrate the applicability of our findings, we reanalyze the data from the Systolic Blood Pressure Intervention Trial (SPRINT) and the Action to Control Cardiovascular Risk in Diabetes (ACCORD) study. While recent literature reports the existence of heterogeneous effects of intensive blood pressure treatment with multiple treatment effect modifiers, our results suggest that many of these modifiers may be spurious discoveries. This chapter is accompanied by survlearners, an R package that provides well-documented implementations of the CATE estimation strategies described in this work, to allow easy use of our recommendations as well as the reproduction of our numerical study.

==> Treatment Heterogeneity for Survival Outcomes/Tables/Table4.tex <==

\begin{table}[ht]
\centering
\caption{Performance assessment of metalearners in CATE estimation via global null analysis. By construction, the true CATEs in the modified SPRINT and ACCORD datasets are zero for all subjects. Original baseline covariates are used. The metalearners showed various amounts of overestimation of treatment heterogeneity (in terms of RMSEs), which may lead to false discoveries. The analysis was repeated for subjects under the standard and intensive arms and replicated to model censoring using a random survival forest and the Kaplan-Meier estimator, separately.}
\label{t:zerocatefull}
\begin{tabular}{cccccccc}
  \hline
   \multicolumn{4}{c}{Standard} & \multicolumn{4}{c}{Intensive}\\ \hline
   \multicolumn{2}{c}{Survival Forest} & \multicolumn{2}{c}{Kaplan-Meier}&\multicolumn{2}{c}{Survival Forest} & \multicolumn{2}{c}{Kaplan-Meier}\\ \hline
   Estimator & RMSE & Estimator & RMSE & Estimator & RMSE & Estimator & RMSE \\ 
  \hline
    \multicolumn{8}{c}{SPRINT}\\ \hline
 SF* & 0.0005 & SF* & 0.0005 & SF* & 0.0003 & SF* & 0.0003 \\ 
  M*L & 0.0008 & M*L & 0.0007 & M*L & 0.0021 & M*L & 0.0017 \\ 
  RFL & 0.0011 & RFL & 0.0015 & RLL & 0.0024 & RFL & 0.0022 \\ 
  RLL & 0.0021 & RLL & 0.0112 & RFL & 0.0027 & RLL & 0.0022 \\ 
  XLL & 0.0085 & XFF & 0.0120 & SL* & 0.0090 & XLL & 0.0088 \\ 
  XFF & 0.0114 & RFF & 0.0123 & XFL & 0.0094 & SL* & 0.0090 \\ 
  RFF & 0.0118 & TF* & 0.0139 & XLL & 0.0127 & XFL & 0.0116 \\ 
  TF* & 0.0139 & CSF & 0.0145 & RFF & 0.0136 & RFF & 0.0137 \\ 
  M*F & 0.0141 & M*F & 0.0145 & TF* & 0.0141 & TF* & 0.0141 \\ 
  CSF & 0.0145 & SL* & 0.0161 & XFF & 0.0146 & CSF & 0.0151 \\ 
  SL* & 0.0161 & XFL & 0.0179 & M*F & 0.0147 & XFF & 0.0152 \\ 
  XFL & 0.0176 & XLL & 0.0205 & CSF & 0.0151 & M*F & 0.0152 \\ 
  TL* & 0.0351 & TL* & 0.0351 & TL* & 0.0280 & TL* & 0.0280 \\ \hline
   \multicolumn{8}{c}{ACCORD-BP}\\ \hline
  SF* & 0.0010 & SF* & 0.0010 & SF* & 0.0013 & SF* & 0.0013 \\ 
  M*L & 0.0103 & M*L & 0.0104 & RLL & 0.0026 & RLL & 0.0027 \\ 
  RFL & 0.0106 & RFL & 0.0108 & RFL & 0.0034 & RFL & 0.0038 \\ 
  RLL & 0.0121 & RLL & 0.0167 & SL* & 0.0047 & SL* & 0.0047 \\ 
  XLL & 0.0132 & XFF & 0.0177 & M*L & 0.0062 & M*L & 0.0065 \\ 
  XFF & 0.0178 & XLL & 0.0189 & XLL & 0.0144 & XLL & 0.0157 \\ 
  TF* & 0.0204 & TF* & 0.0204 & XFL & 0.0283 & XFL & 0.0305 \\ 
  RFF & 0.0212 & RFF & 0.0213 & XFF & 0.0329 & XFF & 0.0320 \\ 
  CSF & 0.0220 & CSF & 0.0220 & CSF & 0.0336 & CSF & 0.0336 \\ 
  M*F & 0.0253 & XFL & 0.0223 & TL* & 0.0338 & TL* & 0.0338 \\ 
  XFL & 0.0265 & M*F & 0.0245 & RFF & 0.0347 & RFF & 0.0346 \\ 
  SL* & 0.0291 & SL* & 0.0291 & TF* & 0.0367 & TF* & 0.0367 \\ 
  TL* & 0.0296 & TL* & 0.0296 & M*F & 0.0438 & M*F & 0.0421 \\ 
   \hline
 \end{tabular}
\end{table}


==> Treatment Heterogeneity for Survival Outcomes/Tables/Table5.tex <==
\begin{table}[ht]
\centering
\caption{Internal and external validation performance of CATE estimation in SPRINT and ACCORD-BP, respectively. For internal validation, none of the five metalearners showed significant AUTOCs, suggesting the lack of treatment heterogeneity of intensive BP therapy. For internal validation, with the original covariates, CSF and XFF showed (marginally) significant AUTOCs. RECETH is the square root of the default calibration error given by ECETH.}
\label{t:sprint_eval}
\resizebox{\textwidth}{!}{\begin{tabular}{lcccc}
 \hline 
       & \multicolumn{2}{c}{Original covariates} & \multicolumn{2}{c}{PCE + CKD}\\ \hline
Method & AUTOC & RECETH & AUTOC & RECETH \\ \hline
  \multicolumn{5}{c}{Internal Validation}\\ \hline
  SL* & -0.0043 (-0.0260, 0.0174)  & 0.0211 (0.0000, 0.0452) & -0.0002 (-0.0223, 0.0218) & 0.0006 (0.0000, 0.0358) \\ 
  TL* & -0.0002 (-0.0206, 0.0202)  & 0.0023 (0.0000, 0.0404) &  0.0002 (-0.0209, 0.0212) & 0.0142 (0.0000, 0.0431) \\ 
  XFF &  0.0048 (-0.0162, 0.0258)  & 0.0135 (0.0000, 0.0386) & -0.0144 (-0.0348, 0.0059) & 0.0186 (0.0000, 0.0426) \\ 
  XFL & -0.0053 (-0.0270, 0.0165)  & 0.0235 (0.0000, 0.0469) & -0.0019 (-0.0232, 0.0195) & 0.0000 (0.0000, 0.0285) \\ 
  RFL &  0.0000 ( 0.0000, 0.0000)  & 0.0142 (0.0000, 0.0307) &  0.0044 (-0.0161, 0.0248) & 0.0000 (0.0000, 0.0301) \\ 
  CSF &  0.0012 (-0.0187, 0.0211)  & 0.0184 (0.0000, 0.0425) & -0.0172 (-0.0371, 0.0028) & 0.0451 (0.0185, 0.0644) \\  \hline
\multicolumn{5}{c}{External Validation}\\ \hline
  SL* & -0.0092 (-0.0281, 0.0097)   & 0.0077 (0.0000, 0.0332) & -0.0031 (-0.0201, 0.0138) & 0.0000 (0.0000, 0.0277) \\ 
  TL* & -0.0100 (-0.0274, 0.0073)   & 0.0242 (0.0000, 0.0421) & -0.0095 (-0.0261, 0.0072) & 0.0215 (0.0000, 0.0406) \\ 
  XFF &  0.0169 (-0.0006, 0.0345)   & 0.0000 (0.0000, 0.0201) & -0.0088 (-0.0261, 0.0085) & 0.0362 (0.0111, 0.0526) \\ 
  XFL & -0.0081 (-0.0254, 0.0091)   & 0.0201 (0.0000, 0.0391) & -0.0095 (-0.0261, 0.0071) & 0.0162 (0.0000, 0.0377) \\ 
  RFL &  0.0000 ( 0.0000, 0.0000)   & 0.0087 (0.0000, 0.0229) &  0.0000 ( 0.0000, 0.0000) & 0.0074 (0.0000, 0.0221) \\ 
  CSF &  0.0178 ( 0.0010, 0.0345)   & 0.0000 (0.0000, 0.0294) & -0.0111 (-0.0282, 0.0060) & 0.0321 (0.0000, 0.0486) \\   \hline
\end{tabular}}
\end{table}

==> Treatment Heterogeneity for Survival Outcomes/Tables/Table6.tex <==
\begin{table}[ht]
\centering
\caption{Performance assessment of metalearners in CATE estimation via global null analysis. By construction, the true CATEs in the modified SPRINT and ACCORD datasets are zero for all subjects. The estimated ten-year CVD risk (using the pooled cohort question) and subclinical CKD are used as predictors. The metalearners showed various amounts of overestimation of treatment heterogeneity (in terms of RMSEs), which may lead to false discoveries. The analysis was repeated for subjects under the standard and intensive arms and replicated to model censoring using a random survival forest and the Kaplan-Meier estimator, separately.}
\label{t:zerocatepce}
\begin{tabular}{cccccccc}
  \hline
   \multicolumn{4}{c}{Standard} & \multicolumn{4}{c}{Intensive}\\ \hline
   \multicolumn{2}{c}{Survival Forest} & \multicolumn{2}{c}{Kaplan-Meier}&\multicolumn{2}{c}{Survival M*orest} & \multicolumn{2}{c}{Kaplan-Meier}\\ \hline
   Estimator & RMSE & Estimator & RMSE & Estimator & RMSE & Estimator & RMSE \\ 
  \hline
    \multicolumn{8}{c}{SPRINT}\\ \hline
  RFL & 0.0001 & RLL & 0.0001 & SL* & 0.0003 & SL* & 0.0003 \\ 
  RLL & 0.0011 & XLL & 0.0006 & RLL & 0.0008 & M*L & 0.0017 \\ 
  M*L & 0.0014 & M*L & 0.0007 & XLL & 0.0014 & SF* & 0.0040 \\ 
  SL* & 0.0027 & RFL & 0.0012 & RFL & 0.0020 & RFL & 0.0053 \\ 
  XFL & 0.0058 & SL* & 0.0027 & M*L & 0.0021 & TL* & 0.0078 \\ 
  XLL & 0.0075 & XFL & 0.0090 & SF* & 0.0040 & TF* & 0.0082 \\ 
  SF* & 0.0098 & SF* & 0.0098 & XFL & 0.0069 & XFL & 0.0086 \\ 
  TL* & 0.0110 & TL* & 0.0110 & TL* & 0.0078 & XLL & 0.0092 \\ 
  TF* & 0.0188 & TF* & 0.0188 & TF* & 0.0082 & RLL & 0.0132 \\ 
  XFF & 0.0214 & XFF & 0.0214 & XFF & 0.0137 & CSF & 0.0155 \\ 
  RFF & 0.0249 & RFF & 0.0243 & CSF & 0.0155 & XFF & 0.0169 \\ 
  CSF & 0.0280 & CSF & 0.0280 & RFF & 0.0167 & M*F & 0.0176 \\ 
  M*F & 0.0360 & M*F & 0.0348 & M*F & 0.0172 & RFF & 0.0187 \\\hline
   \multicolumn{8}{c}{ACCORD-BP}\\ \hline
  SL* & 0.0080 & SL* & 0.0080 & M*L & 0.0057 & RLL & 0.0041 \\ 
  XLL & 0.0096 & RLL & 0.0099 & SL* & 0.0069 & SL* & 0.0069 \\ 
  RLL & 0.0100 & TL* & 0.0104 & SF* & 0.0151 & M*L & 0.0111 \\ 
  TL* & 0.0104 & M*L & 0.0104 & TL* & 0.0190 & SF* & 0.0151 \\ 
  M*L & 0.0106 & RFL & 0.0107 & XLL & 0.0201 & TL* & 0.0190 \\ 
  RFL & 0.0107 & XFL & 0.0108 & XFL & 0.0230 & XLL & 0.0199 \\ 
  XFL & 0.0108 & XLL & 0.0111 & RFL & 0.0243 & RFL & 0.0205 \\ 
  SF* & 0.0117 & SF* & 0.0117 & CSF & 0.0267 & XFL & 0.0248 \\ 
  TF* & 0.0220 & TF* & 0.0220 & RFF & 0.0267 & CSF & 0.0267 \\ 
  XFF & 0.0248 & XFF & 0.0245 & RLL & 0.0282 & RFF & 0.0277 \\ 
  RFF & 0.0287 & CSF & 0.0288 & TF* & 0.0299 & TF* & 0.0299 \\ 
  CSF & 0.0288 & RFF & 0.0293 & M*F & 0.0310 & XFF & 0.0305 \\ 
  M*F & 0.0376 & M*F & 0.0376 & XFF & 0.0314 & M*F & 0.0317 \\ 
   \hline
 \end{tabular}
\end{table}

